Learning Linear Temporal Properties from Noisy Data: A MaxSAT Approach

We address the problem of inferring descriptions of system behavior using Linear Temporal Logic (LTL) from a finite set of positive and negative examples. Most of the existing approaches for solving such a task rely on predefined templates for guiding the structure of the inferred formula. The approaches that can infer arbitrary LTL formulas, on the other hand, are not robust to noise in the data. To alleviate such limitations, we devise two algorithms for inferring concise LTL formulas even in the presence of noise. Our first algorithm infers minimal LTL formulas by reducing the inference problem to a problem in maximum satisfiability and then using off-the-shelf MaxSAT solvers to find a solution. To the best of our knowledge, we are the first to incorporate the usage of MaxSAT solvers for inferring formulas in LTL. Our second learning algorithm relies on the first algorithm to derive a decision tree over LTL formulas based on a decision tree learning algorithm. We have implemented both our algorithms and verified that our algorithms are efficient in extracting concise LTL descriptions even in the presence of noise.

==> charts.tex <==
% !TEX root = main.tex


\FloatBarrier
\subsection{\MaxSAT{} compared to \SAT{}}

We compare \MaxSAT{} (proposed in this paper) and \SAT{} (proposed in \cite{DBLP:conf/fmcad/NeiderG18})
in Figures \ref{app:fig:sat-vs-maxsat:time} and \ref{app:fig:sat-vs-maxsat:LTL}.

\begin{figure*}[h]
\centering
\vspace{-4mm}
%
\begin{subfigure}{.4\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-11a.tex]{
		loglog
		--title 'Benchmark without noise'
		--xlabel '\SAT{} ($s$)' --ylabel '\MaxSAT{}($\thres=0.00$) ($s$)'
		--table joinedByTraces.csv
		--keep-only benchmark_noise:0.0
		--columns runtime_SAT:runtime_MaxSAT0
	}
\end{subfigure}
%\hspace{1.5cm}
\begin{subfigure}{.4\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-11b.tex]{
		loglog
		--title 'Benchmark with 5\% noise'
		--xlabel '\SAT{} ($s$)' --ylabel '\MaxSAT{}($\thres=0.00$) ($s$)'
		--table joinedByTraces.csv
		--keep-only benchmark_noise:0.05
		--columns runtime_SAT:runtime_MaxSAT0
	}
\end{subfigure}

\begin{subfigure}{.4\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-11c.tex]{
		loglog
		--title 'Benchmark without noise'
		--xlabel '\SAT{} ($s$)' --ylabel '\MaxSAT{}($\thres=0.05$) ($s$)'
		--table joinedByTraces.csv
		--keep-only benchmark_noise:0.0
		--columns runtime_SAT:runtime_MaxSAT5
	}
\end{subfigure}
%\hspace{1.5cm}
\begin{subfigure}{.4\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-11d.tex]{
		loglog
		--title 'Benchmark with 5\% noise'
		--xlabel '\SAT{} ($s$)' --ylabel '\MaxSAT{}($\thres=0.05$) ($s$)'
		--table joinedByTraces.csv
		--keep-only benchmark_noise:0.05
		--columns runtime_SAT:runtime_MaxSAT5
	}
\end{subfigure}

\begin{subfigure}{.4\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-11e.tex]{
		loglog
		--title 'Benchmark without noise'
		--xlabel '\SAT{} ($s$)' --ylabel '\MaxSAT{}($\thres=0.10$) ($s$)'
		--table joinedByTraces.csv
		--keep-only benchmark_noise:0.0
		--columns runtime_SAT:runtime_MaxSAT10
	}
\end{subfigure}
%\hspace{1.5cm}
\begin{subfigure}{.4\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-11f.tex]{
		loglog
		--title 'Benchmark with 5\% noise'
		--xlabel '\SAT{} ($s$)' --ylabel '\MaxSAT{}($\thres=0.10$) ($s$)'
		--table joinedByTraces.csv
		--keep-only benchmark_noise:0.05
		--columns runtime_SAT:runtime_MaxSAT10
	}
\end{subfigure}

\caption{
	Running time comparison in seconds of \SAT{} and \MaxSAT{}
	with different values for the threshold $\thres$.
	$900 s$ of running time means that the algorithm timed out.
}
\label{app:fig:sat-vs-maxsat:time}
\vspace{-11mm}
\end{figure*}




\begin{figure*}[h]
\centering

\begin{subfigure}{0.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-12a.tex]{
		bubble
		--title 'Benchmark without noise'
		--xlabel '\SAT{}' --ylabel '\MaxSAT{}($\thres=0.00$)'
		--table SizeFreq-MaxSATvsSAT-timeouts.csv
		--columns SAT-perf1:MaxSAT0-perf:Freq-perf1
	}
\end{subfigure}
%
\begin{subfigure}{0.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-12b.tex]{
		bubble
		--title 'Benchmark with 5\% noise'
		--xlabel '\SAT{}' --ylabel '\MaxSAT{}($\thres=0.00$)'
		--table SizeFreq-MaxSATvsSAT-timeouts.csv
		--columns SAT-noisy1:MaxSAT0-noisy:Freq-noisy1
	}
\end{subfigure}

\begin{subfigure}{0.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-12c.tex]{
		bubble
		--title 'Benchmark without noise'
		--xlabel '\SAT{}' --ylabel '\MaxSAT{}($\thres=0.05$)'
		--table SizeFreq-MaxSATvsSAT-timeouts.csv
		--columns SAT-perf2:MaxSAT5-perf:Freq-perf2
	}
\end{subfigure}
%
\begin{subfigure}{0.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-12d.tex]{
		bubble
		--title 'Benchmark with 5\% noise'
		--xlabel '\SAT{}' --ylabel '\MaxSAT{}($\thres=0.05$)'
		--table SizeFreq-MaxSATvsSAT-timeouts.csv
		--columns SAT-noisy2:MaxSAT5-noisy:Freq-noisy2
	}
\end{subfigure}

\begin{subfigure}{0.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-12e.tex]{
		bubble
		--title 'Benchmark without noise'
		--xlabel '\SAT{}' --ylabel '\MaxSAT{}($\thres=0.10$)'
		--table SizeFreq-MaxSATvsSAT-timeouts.csv
		--columns SAT-perf3:MaxSAT10-perf:Freq-perf3
	}
\end{subfigure}
%
\begin{subfigure}{0.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-12f.tex]{
		bubble
		--title 'Benchmark with 5\% noise'
		--xlabel '\SAT{}' --ylabel '\MaxSAT{}($\thres=0.10$)'
		--table SizeFreq-MaxSATvsSAT-timeouts.csv
		--columns SAT-noisy3:MaxSAT10-noisy:Freq-noisy3
	}
\end{subfigure}

\caption{
	Inferred \LTLf{} formula size comparison of \SAT{} and \MaxSAT{}
	with different values for the threshold $\thres$.
	The surface of the dots is proportional to the number of samples represented.
	We denote \LTLf{} formula not inferred because of timeouts by $\emptyset$.
}
\label{app:fig:sat-vs-maxsat:LTL}
\end{figure*}


\FloatBarrier
\subsection{\MaxSATDT{} compared to \MaxSAT{}}

We compare \MaxSATDT{} to \MaxSAT{} (both proposed in this paper) in Figure \ref{app:fig:maxsat-vs-maxsatdt}.


\begin{figure*}[h]
\centering
%
\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-21a.tex]{
		loglog
		--title 'Running time in $s$'
		--xlabel '\MaxSAT{}' --ylabel '\MaxSATDT{}($\minscore=0.80$)'
		--table joinedByTraces.csv
		--columns runtime_MaxSAT5:runtime_MaxSATDT80
		--min=1e-3 %--max=1e3
	}
\end{subfigure}
%\hspace{1.5cm}
\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-21b.tex]{
		loglog
		--title 'Inferred \LTLf{} formula size'
		--xlabel '\MaxSAT{}' --ylabel '\MaxSATDT{}($\minscore=0.80$)'
		--table joinedByTraces.csv
		--columns LTL_size_MaxSAT5:LTL_size_MaxSATDT80
		--min=1 --max=250
	}
\end{subfigure}

\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-21c.tex]{
		loglog
		--title 'Running time in $s$'
		--xlabel '\MaxSAT{}' --ylabel '\MaxSATDT{}($\minscore=0.60$)'
		--table joinedByTraces.csv
		--columns runtime_MaxSAT5:runtime_MaxSATDT60
		--min=1e-3 %--max=1e3
	}
\end{subfigure}
%\hspace{1.5cm}
\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-21d.tex]{
		loglog
		--title 'Inferred \LTLf{} formula size'
		--xlabel '\MaxSAT{}' --ylabel '\MaxSATDT{}($\minscore=0.60$)'
		--table joinedByTraces.csv
		--columns LTL_size_MaxSAT5:LTL_size_MaxSATDT60
		--min=1 --max=250
	}
\end{subfigure}

\caption{
	Comparison on all benchmarks of the performances of \MaxSATDT{}($\minscore$) and \MaxSAT{},
	with $\thres=0.05$ for both algorithms.
	$900 s$ of running time means that the algorithm timed out.
}
\label{app:fig:maxsat-vs-maxsatdt}
\end{figure*}




\clearpage
\FloatBarrier
\subsection{\MaxSATDT{} performances in function of $\minscore$ parameter}

We evaluate the effects of $\minscore$ parameter on \MaxSATDT{} (proposed in this paper)
in Figure \ref{app:fig:maxsatdt}

\begin{figure*}[h]
\centering
%
\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-31a.tex]{
		loglog
		--title 'Running time in $s$'
		--xlabel '\MaxSATDT{}($\minscore=0.80$' --ylabel '\MaxSATDT{}($\minscore=0.60$)'
		--table joinedByTraces.csv
		--columns runtime_MaxSATDT80:runtime_MaxSATDT60
		--min=1e-3 %--max=1e3
	}
\end{subfigure}
%\hspace{1.5cm}
\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-31b.tex]{
		loglog
		--title 'Inferred \LTLf{} formula size'
		--xlabel '\MaxSATDT{}($\minscore=0.80$' --ylabel '\MaxSATDT{}($\minscore=0.60$)'
		--table joinedByTraces.csv
		--columns LTL_size_MaxSATDT80:LTL_size_MaxSATDT60
		--min=1 --max=250
	}
\end{subfigure}

\caption{
	Comparison on all benchmarks of the performances of \MaxSATDT{}($\minscore$)
	with respectively $\minscore=0.80$ and $\minscore=0.60$.
	$\thres$ is set to $0.05$.
	$900 s$ of running time means that the algorithm timed out.
}
\label{app:fig:maxsatdt}
\end{figure*}



\clearpage
\FloatBarrier
\subsection{\MaxSATDT{} compared to \SATDT{}}

We compare \MaxSATDT{} (proposed in this paper) and \SATDT{} (proposed in \cite{DBLP:conf/fmcad/NeiderG18})
in Figure \ref{app:fig:satdt-vs-maxsatdt}.

\begin{figure*}[h]
\centering
%
\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-41a.tex]{
		loglog
		--title 'Running time in $s$'
		--xlabel '\SATDT{}' --ylabel '\MaxSATDT{}($\minscore=0.80$)'
		--table joinedByTraces.csv
		--columns runtime_SATDT:runtime_MaxSATDT80
		--min=1e-3 %--max=1e3
	}
\end{subfigure}
%\hspace{1.5cm}
\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-41b.tex]{
		loglog
		--title 'Inferred \LTLf{} formula size'
		--xlabel '\SATDT{}' --ylabel '\MaxSATDT{}($\minscore=0.80$)'
		--table joinedByTraces.csv
		--columns LTL_size_SATDT:LTL_size_MaxSATDT80
		--min=1 --max=250
	}
\end{subfigure}

\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-41c.tex]{
		loglog
		--title 'Running time in $s$'
		--xlabel '\SATDT{}' --ylabel '\MaxSATDT{}($\minscore=0.60$)'
		--table joinedByTraces.csv
		--columns runtime_SATDT:runtime_MaxSATDT60
		--min=1e-3 %--max=1e3
	}
\end{subfigure}
%\hspace{1.5cm}
\begin{subfigure}{.45\linewidth}
	\centering
	\includepgfgenerate[fig-app-eval-41d.tex]{
		loglog
		--title 'Inferred \LTLf{} formula size'
		--xlabel '\SATDT{}' --ylabel '\MaxSATDT{}($\minscore=0.60$)'
		--table joinedByTraces.csv
		--columns LTL_size_SATDT:LTL_size_MaxSATDT60
		--min=1 --max=250
	}
\end{subfigure}

\caption{
	Comparison on all benchmarks of the performances of \MaxSATDT{}($\minscore$) and \SATDT{},
	with $\thres=0.05$ for both algorithms.
	$900 s$ of running time means that the algorithm timed out.
}
\label{app:fig:satdt-vs-maxsatdt}
\end{figure*}

